Trust Regions for Explanations via Black-Box Probabilistic Certification

Given the black box nature of machine learning models, a plethora of explainability methods have been developed to decipher the factors behind individual decisions. In this paper, we introduce a novel problem of black box (probabilistic) explanation certification. We ask the question: Given a black box model with only query access, an explanation for an example and a quality metric (viz. fidelity, stability), can we find the largest hypercube (i.e., $\ell_{\infty}$ ball) centered at the example such that when the explanation is applied to all examples within the hypercube, (with high probability) a quality criterion is met (viz. fidelity greater than some value)? Being able to efficiently find such a \emph{trust region} has multiple benefits: i) insight into model behavior in a \emph{region}, with a \emph{guarantee}; ii) ascertained \emph{stability} of the explanation; iii) \emph{explanation reuse}, which can save time, energy and money by not having to find explanations for every example; and iv) a possible \emph{meta-metric} to compare explanation methods. Our contributions include formalizing this problem, proposing solutions, providing theoretical guarantees for these solutions that are computable, and experimentally showing their efficacy on synthetic and real data.

==> extra.tex <==
\subsection{Certifying a Given Explanation}

In this first problem, we are given a predictive model $g(\vx)$, $g: \R^d \to \R$, and a point of interest $\vx_0 \in \R^d$. We are also given a local explanation $e_{\vx_0}(\vx)$ of $g(\vx)$ at the point $\vx_0$ and a non-negative loss function $\ell(e_{\vx_0}(\vx), g(\vx))$ that measures the error of $e_{\vx_0}(\vx)$ in approximating $g(\vx)$. In one formulation, our goal is to find the worst loss (i.e., largest error) within a given region $R$ containing $\vx_0$:
\begin{equation}\label{eq:fixedRegion}
    \max_{\vx\in R} \; \ell(e_{\vx_0}(\vx), g(\vx)).
\end{equation}
In this work, we take $R$ to be an $\ell_\infty$ ball $B_\infty(\vx_0, \epsilon)$ of radius $\epsilon$ centered at $\vx_0$.

Alternatively, we may be given an upper bound $\theta$ on the acceptable loss and wish to find the largest ball such that the loss everywhere within the ball is no greater than $\theta$:
\begin{equation}\label{eq:fixedThresh}
    \max \quad r \quad \text{s.t.} \quad \ell(e_{\vx_0}(\vx), g(\vx)) \leq \theta \quad \forall \vx \in B_\infty(\vx_0, r).
\end{equation}
If we have an algorithm for problem \eqref{eq:fixedRegion}, then we may use it along with a search over $r$ to solve \eqref{eq:fixedThresh}: Given $r$ and $B_\infty(\vx_0, r)$, the algorithm for \eqref{eq:fixedRegion} is used to check whether the constraint in \eqref{eq:fixedThresh} holds for all $\vx \in B_\infty(\vx_0, r)$ (i.e., whether it holds for the maximum). If the constraint is satisfied, then we increase $r$, and otherwise decrease it.

[discuss difficulty of $R$ being an uncountably infinite set]

\subsection{Obtaining an Explanation with the Best Certificate}

In the second problem that we consider, rather than certifying a given explanation, we wish to obtain an explanation that minimizes the maximum loss in \eqref{eq:fixedRegion}. For this, we restrict attention to linear explanation functions $e_{\vx_0}(\vx) = \valpha^T \vx$. The problem is therefore  
\begin{equation}\label{eq:minimax}
    \min_{\valpha} \; \max_{\vx\in R} \; \ell(\valpha^T \vx, g(\vx)).
\end{equation}

NRK: Perhaps this is obvious, but one of the novel things here is that we are not computing explanation for a point per se, but rather for a region as a whole. This is particularly true if $\ell$ is infinity norm.

\begin{prop}
Problem~\eqref{eq:minimax} is a convex optimization problem if the loss function $\ell(e, g)$ is convex in $e$ for all $g$.
\end{prop}
\begin{proof}
\end{proof}

Although \eqref{eq:minimax} is in theory a convex optimization, its objective function is difficult to compute as discussed above. Thus as an approximation to \eqref{eq:minimax}, we consider a version in which the uncountably infinite set $R$ is replaced by a finite set of samples $\vx_1,\dots,\vx_n$ from $R$. We write this approximate problem by first rewriting \eqref{eq:minimax} in the following equivalent form: 
\begin{equation}\label{eq:minimaxCons}
    \min_{\valpha, t} \quad t \quad \text{s.t.} \quad \ell(\valpha^T \vx, g(\vx)) \leq t \quad \forall \vx \in R.
\end{equation}
We then drop the constraint for all $\vx$ except $\vx_1,\dots,\vx_n$, yielding
\begin{equation}\label{eq:minimaxFinite}
    \min_{\valpha, t} \quad t \quad \text{s.t.} \quad \ell(\valpha^T \vx_i, g(\vx_i)) \leq t \quad i=1,\dots,n.
\end{equation}
Since \eqref{eq:minimaxFinite} has fewer constraints, the optimal value in \eqref{eq:minimaxFinite} is a lower bound on that in \eqref{eq:minimaxCons}.

We now propose to solve \eqref{eq:minimaxCons} by solving \eqref{eq:minimaxFinite} and using \emph{constraint generation}. The basic procedure is as follows:
\begin{enumerate}
    \item Solve \eqref{eq:minimaxFinite} for a set of samples $\vx_1,\dots,\vx_n$ to obtain an optimal solution $\valpha^*$ and optimal value (minimax loss) $t^*$.
    \item Solve \eqref{eq:fixedRegion} with $e_{\vx_0}(\vx) = \valpha^{*T} \vx$ to search for $\vx \in R$ for which the loss exceeds $t^*$.
    \item If an $\vx$ is found such that $\ell(\valpha^{*T} \vx, g(\vx)) > t^*$, set $\vx_{n+1} = \vx$ and repeat step 1 with $\vx_1,\dots,\vx_{n+1}$. Otherwise, terminate because $(\valpha^*, t^*)$ is also optimal for \eqref{eq:minimaxCons}.
\end{enumerate}

==> piecewise_linear_old.tex <==
\noindent\textbf{1) Piecewise Linear Black Box Case:}
We characterize the cdfs $F_i(.)$ for a piecewise linear black box function (viz. Oblique trees, Deep Relu Networks, etc.) $g(.):\mathcal{R}^d\rightarrow [0,1]$ and a linear explanation function $e_{\bm{y}}(.):\mathcal{R}^d\rightarrow [0,1]$, where the subscript $\bm{y}$ denotes that the explanation function was estimated at $\bm{y}\in \mathcal{R}^d$, and given the following fidelity function \cite{ans,mame}:
\begin{align}
\label{eq:fid}
    f_{\vy}(\bm{x}) \triangleq 
     1-|g(\bm{x})-e_{\bm{y}}(\bm{x})|
\end{align}
For the unifI and adaptI strategies the cdf functions $F_i^{\mathcal{N}_{j,k}}(.)$ are transformations of normally distributed data with the corresponding prototypes as the mean and variance $\sigma^2$. In the $i^{\text{th}}$ region assume that the black box has $t\le p$ linear pieces present, then the density in that region will be a mixture of $t$ densities one corresponding to each linear piece. Thus, the overall cdf will be determined by these densities. Let us derive what the density will be for some piece $s\le t$ in this region. Let the explanation function be linear and represented by $e_{\bm{y}}(\bm{x})=\sum_{l=1}^d\alpha_{y,l}x_l$ and the $s^{\text{th}}$ black box linear piece be represented by $g_s(\bm{x}) = \sum_{l=1}^d\beta_{s,l}x_l$. Thus, $
\label{eq:diff}
\Delta_s(\bm{x})=g_s(\bm{x})-e_{\bm{y}}(\bm{x}) = \sum_{l=1}^d(\beta_{s,l}-\alpha_{y,l})x_l$.

Now if the sampling density in the input space was based off on prototype $\bm{\mu}$ which would then be its mean, we would have each $x_l\sim \mathcal{N}(\mu_l,\sigma^2)$ and hence, 
$
\Delta_s(\bm{x})\sim \mathcal{N}\left(\sum_{l=1}^d(\beta_{s,l}-\alpha_{y,l})\mu_l,\sigma^2d\right)$. If we take the absolute value of $\Delta_s(x)$ then the distribution will be a folded normal given by,
\begin{align}
\label{eq:Gdistabs}
|\Delta_s(\bm{x})|&\sim \mathcal{N}\left(\sum_{l=1}^d(\beta_{s,l}-\alpha_{y,l})\mu_l,\sigma^2d\right)+\mathcal{N}\left(-\sum_{l=1}^d(\beta_{s,l}-\alpha_{y,l})\mu_l,\sigma^2d\right)=\mathcal{N}^+(\mu_{s+},\sigma_{s+}^2)
\end{align}
where, $\mathcal{N}^+$ implies folded normal distribution with mean
$\mu_{s+}=\sigma\sqrt{\frac{2d}{\pi}}\exp{-\frac{(\sum_{l=1}^d(\beta_{s,l}-\alpha_{y,l})\mu_l)^2}{2\sigma^2d}}+\sum_{l=1}^d(\beta_{s,l}-\alpha_{y,l})\mu_l\text{erf}\left(\frac{\sum_{l=1}^d(\beta_{s,l}-\alpha_{y,l})\mu_l}{\sigma\sqrt{2d}}\right)$ and variance $\sigma_{s+}^2=\sum_{l=1}^d(\beta_{s,l}-\alpha_{y,l})\mu_l+\sigma^2d-\mu_{s+}^2$. erf(.) denotes the Gauss error function. Hence, the density of the fidelity function corresponding to the $s^{th}$ piece would be,
\begin{align}
    \label{eq:dens}
    1-|\Delta_s(\bm{x})|\sim \mathcal{N}^+(1-\mu_{s+},\sigma_{s+}^2)
\end{align}
The cdfs $F_i^{\mathcal{N}_{j,k}}(.)$ associated with each prototype indexed by $(j,k)$ would be over $t$ such densities where $s\in\{1,...,t\}$ and only one of these densities corresponding to the linear piece of the black box would be active at any point in time for a region $i$.

For the unif case we could follow similar steps where rather than normally distributed independent random variables we would have have uniformly distributed ones with different ranges. However, in this case it is challenging to come up with an expression like in the above one, since uniform distributions have sharp cutoffs and the resultant distributions are non-smooth with typically the number of separate functions equal to the number of uniform random variables being added\footnote{If the variables were i.i.d. $U(0,1)$ we would obtain the (non-smooth) Irwin-Hall distribution.}. Asymptotically of course given that the uniforms are independent certain generalizations of the Central limit theorem (CLT) may be applicable such as Lindeberg CLT noting that the distribution of the sum of these variables will converge to a normal distribution. Then taking absolute value, negating and adding 1 should give again a folded normal distribution that is reflected about the origin and shifted by 1 as before but with its corresponding mean and variance parameters.

